Entropic Independence I: Modified Log-Sobolev Inequalities for Fractionally Log-Concave Distributions and High-Temperature Ising Models

We introduce a notion called entropic independence that is an entropic analog of spectral notions of high-dimensional expansion. Informally, entropic independence of a background distribution $\mu$ on $k$-sized subsets of a ground set of elements says that for any (possibly randomly chosen) set $S$, the relative entropy of a single element of $S$ drawn uniformly at random carries at most $O(1/k)$ fraction of the relative entropy of $S$. Entropic independence is the analog of the notion of spectral independence, if one replaces variance by entropy. We use entropic independence to derive tight mixing time bounds, overcoming the lossy nature of spectral analysis of Markov chains on exponential-sized state spaces. In our main technical result, we show a general way of deriving entropy contraction, a.k.a. modified log-Sobolev inequalities, for down-up random walks from spectral notions. We show that spectral independence of a distribution under arbitrary external fields automatically implies entropic independence. To derive our results, we relate entropic independence to properties of polynomials: $\mu$ is entropically independent exactly when a transformed version of the generating polynomial of $\mu$ is upper bounded by its linear tangent; this property is implied by concavity of the said transformation, which was shown by prior work to be locally equivalent to spectral independence. We apply our results to obtain tight modified log-Sobolev inequalities and mixing times for multi-step down-up walks on fractionally log-concave distributions. As our flagship application, we establish the tight mixing time of $O(n\log n)$ for Glauber dynamics on Ising models whose interaction matrix has eigenspectrum lying within an interval of length smaller than $1$, improving upon the prior quadratic dependence on $n$.

==> induction.tex <==
\section{Non-uniform Frac LC $\Rightarrow$ MLSI} 
Let $f(x) = x \log x$

For $X_1, \dots, X_n \in \set*{-1,1}^n$ let $\mu(X_1, \dots, X_n) \propto \exp(\frac{1}{2} \langle x, J x\rangle + \langle h, x\rangle )$

Let $\nu$ be arbitrary distribution over $ \set*{-1,1}.$ View $\mu, \nu$ as homogeneous distribution over $\binom{2n}{n}.$

Take $J = u^\intercal u$ with $\norm{u}_2 <1. $

For $X_1, \dots, X_i \in \set*{-1,1}^i$ let
\[\mu(X_1, \dots, X_i) = \sum_{X_{i+1}, \dots,X_n \in \set*{-1,1}^{n-i}} \mu(X_1, \dots, X_i,X_{i+1},\dots, X_n) \]

Similarly define $\nu(X_1, \dots, X_i).$ Let $t(X_1, \dots, X_i) = \frac{\nu(X_1, \dots, X_i)}{\mu(X_1, \dots, X_i)}.$

\[\Delta(X_1, \dots, X_i)  = f\circ t (X_1, \dots, X_i) - f \circ t (X_1,\dots, X_{i-1}) \]

\[d_i = E_{X_1, \dots, X_i}[\Delta(X_1, \dots, X_i)] = \sum \mu(X_1, \dots, X_i) \Delta(X_1, \dots, X_i)\]
\begin{comment}
Suppose we can show
\[(1- \frac{1}{n (1- \norm{u}^2) })(d_n + \dots + d_1 ) \geq d_{n-1} + \dots +d_1\]

then
\[ (1- \frac{1}{n (1- \norm{u}^2) })d_n \geq \frac{1}{n (1- 
\norm{u}^2) }(d_{n-1} + \dots +d_1) \]
\begin{equation} \label{ineq: n vs 1}
(n (1- \norm{u}^2)  -1 ) d_n \geq  (d_{n-1} + \dots +d_1)
\end{equation}
Suppose we can show this for $\mu( \cdot \mid X_n = 1).$ Then \cref{ineq: n vs 1} becomes %then in above inn just replace $ \norm{u} $ by $\norm{u_{-i}}.$
\begin{equation}
\begin{split}
    ((n-1) (1- \norm{u_{-n}}^2)-1) &\sum_{X_1, \dots, X_{n-1}} \mu(X_1, \dots, X_{n-1}, 1) (f \circ t (X_1, \dots, X_{n-1},1) - f\circ t (X_1, \dots, X_{n-2},\cdot, 1))
    \\
    &\geq \D{\nu(\cdot \mid X_n =1) D \mid \mu(\cdot \mid X_n=1) D}
\end{split}
\end{equation}
We take average over all $X_i$ taking value in $\set*{\pm 1}.$ For each $ x_1, \dots, x_n \in \set*{\pm 1}^n$ the coefficient associated with $ \mu(x_1, \dots, x_n) f \circ t (x_1, \dots, x_n)$ is
\[ n-2 - (n-1) \frac{\sum_{i=1}^n \norm{u_{-i}}^2 }{n}) = n-2 - \frac{(n-1)^2}{n} \norm{u}^2 \leq (n-2) (1- \norm{u}^2 ) \]
the coefficient associated with $ \mu(x_1, \dots, x_{n-1}) f \circ t (x_1, \dots, x_{n-1}, \cdot)$ is
\[-(n-2 - (n-1)\frac{\sum_{i=1}^{n-1}\norm{u_{-i}}^2}{n-1}) = -(n-2) + ((n-1) u_n^2 + (n-2) \sum_{i=1}^{n-1} u_i^2)= u_n^2 - (n-2) (1 - \norm{u}^2)  
%(n-2) (1- \norm{u}^2)
\]
If we can get 
\[(n-2) (1- \norm{u}^2) d_n \geq d_{n-1} + \dots +d_2\]
then
\[ (n-2) (1- \norm{u}^2)  ( d_n + \dots + d_2) \geq ( 1+  (n-2) (1- \norm{u}^2)) ( d_{n-1} + \dots +d_2) \]
if we have
\[(d_n + \dots + d_1) \geq r d_1\]
then
\[d_n ((n-2) (1- \norm{u}^2) +1) \geq d_n + \dots + d_2 \geq (r  -1) d_1 \]
thus 
\[((n-2) (1- \norm{u}^2)\frac{r}{r-1} +\frac{1}{r-1}) d_n \geq d_{n-1} + \dots + d_2 + d_1 \]
For \[((n-2) (1- \norm{u}^2)\frac{r}{r-1} +\frac{1}{r-1}) \leq n (1- \norm{u}^2)  -1 \]
we need
\[ (n(1- \norm{u}^2) -1 - (n-2) (1- \norm{u}^2) )r \geq 1 + n (1- \norm{u}^2)  -1  \]
\[(1- 2 \norm{u}^2) r \geq n(1-\norm{u}^2)\]
must be false with $\norm{u} > 1/2.$
\end{comment}
Goal (induction hypothesis), for constant $C > 0$:
\begin{equation}\label{ineq:induction hypothesis}
    (1- \frac{1- \norm{u}^2}{C n  }) \D{\nu \given \mu} \geq \D{\nu D \given \mu D}
\end{equation}
%\[(1- \frac{1- \norm{u}^2}{C n  })(d_n + \dots + d_1 ) \geq d_{n-1} + \dots +d_1\]
Suppose we can show this for $\mu( \cdot \mid X_n = 1).$ Then %\cref{ineq: n vs 1} becomes %then in above inn just replace $ \norm{u} $ by $\norm{u_{-i}}.$
\begin{equation}
\begin{split}
    (1- \frac{1- \norm{u_{-n}}^2}{C(n -1) }) &\sum_{X_1, \dots, X_{n-1}} \mu(X_1, \dots, X_{n-1}, 1) (f \circ t (X_1, \dots, X_{n-1},1) - f\circ t (X_n= 1))
    \\
    &\geq \D{\nu(\cdot \mid X_n =1) D \mid \mu(\cdot \mid X_n=1) D} \\
    &=\frac{1}{n-1} \sum_{i=1}^{n-1} \sum_{x_1, \dots, x_{i-1}, x_{i+1}, x_{n-1}} \mu(X_j = x_j\forall j\neq i, X_n=1) (f \circ t (X_j = x_j\forall j\neq i, X_n=1) - f\circ t (X_n= 1))\\
\end{split}
\end{equation}
thus
\begin{multline}
(1- \frac{1- \norm{u_{-n}}^2}{C(n -1) }) \sum_{X_1, \dots, X_{n-1}} \mu(X_1, \dots, X_{n-1}, 1) f \circ t (X_1, \dots, X_{n-1},1) + \frac{1- \norm{u_{-n}}^2}{C(n -1) } \mu(X_n= 1) f\circ t (X_n=  1) \\
\geq \frac{1}{n-1}\sum_{i=1}^{n-1} \sum_{x_1, \dots, x_{i-1}, x_{i+1}, x_{n-1}} \mu(X_j = x_j\forall j\neq i, X_n=1) f \circ t (X_j = x_j\forall j\neq i, X_n=1)  
\end{multline}
We take sum over all $X_i$ taking value in $\set*{\pm 1},$ then divide by $1/n.$ For each $ x_1, \dots, x_n \in \set*{\pm 1}^n$ the coefficient associated with $ \mu(x_1, \dots, x_n) f \circ t (x_1, \dots, x_n)$ is
\[ \frac{1}{n} \sum_{i=1}^n (1- \frac{1- \norm{u_{-i}}^2}{C(n -1) })  = 1-  \frac{n - (n-1) \norm{u}^2 }{C(n-1)n} = 1 - \frac{1}{C(n-1)} + \frac{\norm{u}^2}{Cn}\]
For $X_{-i} = (x_j)_{j\neq i}$ the coefficient associated with $\mu(X_{-i}) f \circ t(X_{-i})$ is $\frac{n-1}{n}$ 
thus
\begin{multline}
   ( 1 - \frac{1}{C(n-1)} + \frac{\norm{u}^2}{Cn}) \sum_{X_1, \dots, X_{n}} \mu(X_1, \dots, X_{n}) f \circ t (X_1, \dots, X_{n}) + \frac{1}{n}\sum_{i=1}^n  \frac{1- \norm{u_{-i}}^2}{C(n -1) } \mu(X_i= \pm 1) f\circ t (X_i= \pm 1)\\
   \geq %\frac{n-1}{n} 
   \frac{1}{n-1} \cdot \frac{n-1}{n}\sum_{i=1}^n \sum_{(x_j)_{j\neq i}} \mu(X_j = x_j\forall j) f\circ t (X_j = x_j \forall j)
\end{multline}
where $ \mu (X_n = 1) = \sum_{X_{-n}} \mu(X_1, \dots, X_{n-1}, 1). $ (this is because the complex at the link $X_n  = 1$ is 1 dimension less) 

If we can show
\begin{equation} \label{ineq:entropy contraction}
   \sum_{i=1}^n  (1- \norm{u_{-i}}^2) \mu(X_i=\pm 1) f\circ t (X_i= \pm 1) \leq \sum_{X_1, \dots, X_{n}} \mu(X_1, \dots, X_{n}) f \circ t (X_1, \dots, X_{n}) 
\end{equation}
then we are done, since $ - \frac{1}{C(n-1)} + \frac{1}{Cn(n-1)} = -\frac{1}{Cn}.$ Note that the constant $C$ only matter for the base case ($n=2$) but not the induction step. We still need to prove base case though. It only follow from \cref{ineq:entropy contraction} if $ \norm{u}^2 \leq 1/2. $ %and the base case follow from \cref{ineq:entropy contraction} if we set $C = $.

Note: the "orthodox" entropy contraction has $\mu(X_i=1)$ be defined as $1/n$ the current def, and multiply the LHS of  \cref{ineq:entropy contraction} by $n$. The end result is same.

Let $\alpha_i =  (1- \norm{u_{-i}}^2) .$ Let $g(x_1,\dots, x_n, x_{\bar{1}}, \dots, x_{\bar{n}})$ be the homogeneous generating function. If we can prove
\[\log g(x_1^{\alpha_1}, \dots, x_n^{\alpha_n}, x_{\bar{1}}^{\alpha_1}, \dots, x_{\bar{n}}^{\alpha_n})\] is concave for all $\vec{x} \in \R_{\geq 0}^{2n}$ then we are done.


==> multi_spin.tex <==
\section{Multi-spin systems}\label{sec:multispin}
\begin{theorem} \label{thm:multi spin}
Consider matrix $J \in \R^{n\times n}$ such that  $0 \preceq J \preceq I.$
For $i \in [n],$ let $\mathcal{Q}_i $ be an arbitrary distribution on $ S^{d-1}.$ 
Let $\mu$ be the distribution over $S^{d-1}$ with p.d.f.
\[ d \mu(x_1, \dots, x_n) \propto e^{\sum_{i<j} J_{i,j} \langle x_i, x_j \rangle } d Q_1(x_1) \cdots d Q_n(x_n) \]
Then  Glauber dynamics for $\mu$ has KL-contraction $\geq \frac{1 - \norm{u}_2^2}{n}$ and the Glauber dynamics to sample from $\mu$ mixes in $O(n \log n)$ steps. 
\end{theorem}

As in the proof of \cref{thm:main}, Theorem \cref{thm:multi spin} follows from \cref{lem:multi spin} below giving the result in the case of rank-$1$ interaction matrix, upon an (obvious) generalization of \cref{cor:needle}.

\begin{lemma} \label{lem:multi spin}
%\Vishesh{Theorem statement for this section}
Let vector $u \in \R^{n}$ with $\norm{u}_2 \leq 1$ and $J = u u^\intercal.$
For $i \in [n],$ let $\mathcal{Q}_i $ be an arbitrary distribution on $ S^{d-1}.$ 
Let $\mu$ be the distribution over $S^{d-1}$ with p.d.f.
\[ d \mu(x_1, \dots, x_n) \propto e^{\sum_{i<j} J_{i,j} \langle x_i, x_j \rangle } d \mathcal{Q}_1(x_1) \cdots d \mathcal{Q}_n(x_n) \]
Then  Glauber dynamics for $\mu$ has KL-contraction $\geq \frac{1 - \norm{u}_2^2}{n}.$ 
\end{lemma}

For simplicity of notation, we prove the theorem in the case where the distributions $\mathcal{Q}_i$ have finite support. The arguments generalize in a straighforward way to arbitrary $\mathcal{Q}_i$.

%Indeed, any distribution on $S^{d-1}$ can be approximated by a distribution over finite set of points $Q_i \subseteq S^{d-1}$ via an $\epsilon$-net argument.

Suppose $\supp (\mathcal{Q}_i) \subseteq Q$ for some finite set $Q \subseteq S^{d-1}$
We need to bound the entries of the Dobrushin matrix for $\lambda \ast \mu$ for all tilts $\lambda = (\lambda_{i,x})_{i\in [n], x\in Q}.$ To do so, we use the following proposition.
%\June{this prop establish Dobrushin}
\begin{proposition} \label{prop:Dobrushin}
Let $J$ be in $ [-1/\kappa, 1/\kappa].$ 
%Let $\lambda: S^{n-1} \to \R_{\geq 0}.$ Let $u,v  $
Fix a finite set $Q \subseteq S^{d-1}$ and  $\vec{\lambda}\in \R^Q.$ 
%For $v \in \set*{a,b}$, 
For any $v \in S^{n - 1}$, let the distribution $\mu^v:Q \to \R_{\geq 0} $ be defined by $\mu^v(x) \propto \lambda_x e^{J \langle x, v \rangle}.$ Then for any $a, b \in \R^{n-1}$ with $\|a-b\| \le 2\kappa$,
\[ d_{\TV} (\mu^a , \mu^b) \leq \kappa \abs{J}\]
 \end{proposition}
 \begin{comment}
 \begin{proof}
 For $v \in S^{d-1},$ let $Z_v = \sum_{x\in Q} \lambda_x e^{J \langle x, v \rangle}$ be the normalizing constant for $\mu^v.$
 
 Note that by definition of $d_{\TV},$ we only need to prove that for all $Q' \subseteq Q:$
 \[\sum_{x \in Q'} (\mu^a(x) - \mu^b(x)) \leq \abs{J}\]
 Multiply both sides by $Z_a Z_b \geq 0,$ we get the inequality
 \[\sum_{x \in Q'} (\mu^a(x) Z_b - \mu^b(x) Z_a) \leq \abs{J} Z_a Z_b\]
 Fix arbitrary $x \in Q.$
 Since the function $\sum_{x \in Q'} (\mu^a(x) Z_b - \mu^b(x) Z_a) - \abs{J} Z_a Z_b$ is linear in term of $r_{a,x} = e^{J\langle x, a \rangle},$ it is maximizes on the boundary of $r_{a,x}$ i.e. when $r_{a,x} \in \set*{e^J, e^{-J}}.$ Thus, it is enough to show
 the inequality when $\langle x, v\rangle = \pm 1$ for all $x\in Q$ and $v\in \set*{a, b}.$ By grouping the $x$ with same $\langle x, v\rangle$ together, We can rewrite the inequality as
 \begin{equation}\label{ineq:dobrushin edge case}
   \sum_{i=1}^4\abs{\phi_i e^{J \hat{a}_i } Z_b  - \phi_i e^{J \hat{b}_i}Z_a}  \leq 2 \abs{J}Z_a Z_b   
 \end{equation}
 with $\hat{a} = \begin{bmatrix} 1 & 1 & -1 & -1 \end{bmatrix}, \hat{b} = \begin{bmatrix} 1 & -1 & 1 & -1 \end{bmatrix},$ and $\phi_i \geq 0 $ be some functions of $\lambda.$ By replacing $J$ with $-J,$ we only do a permutation of $\set*{\phi_i},$ so we can assume w.l.o.g. that $J \geq 0.$ By exchanging $\hat{a}$ and $\hat{b},$ we can exchange the role of $\phi_2$ and $\phi_3$, so w.l.o.g. we an assume $\phi_2 \leq \phi_3.$ Note that

 \begin{align*}
 &\phi_1 e^{J \hat{a}_1 } Z_b  - \phi_1 e^{J \hat{b}_1}Z_a \\
     &= \phi_1\parens*{ e^J ( \phi_1 e^J + \phi_2 e^{-J} + \phi_3 e^{J} + \phi_4 e^{-J} ) -  e^{J} ( \phi_1 e^J + \phi_2 e^{J} + \phi_3 e^{-J} + \phi_4 e^{-J} ) }\\
     &= \phi_1 \parens*{\phi_2(1 - e^{2J}) + \phi_3 (e^{2J} -1) }\\
     &=\phi_1 (e^{2J}-1) (\phi_3 - \phi_2) \geq 0
     \end{align*}
     \begin{align*}
     &\phi_2 e^{J \hat{a}_2 } Z_b  - \phi_2 e^{J \hat{b}_2}Z_a \\
     &= \phi_2\parens*{ e^J ( \phi_1 e^J + \phi_2 e^{-J} + \phi_3 e^{J} + \phi_4 e^{-J} ) -  e^{-J} ( \phi_1 e^J + \phi_2 e^{J} + \phi_3 e^{-J} + \phi_4 e^{-J} ) }\\
     &=  \phi_2 \parens*{\phi_1 (e^{2J}-1)  +\phi_3 (e^{2J} - e^{-2J}) + \phi_4 (1- e^{-2J}) }\geq 0
     \end{align*}
     \begin{align*}
      &\phi_3 e^{J \hat{a}_3 } Z_b  - \phi_1 e^{J \hat{b}_3}Z_a \\
     &= \phi_3\parens*{ e^{-J} ( \phi_1 e^J + \phi_2 e^{-J} + \phi_3 e^{J} + \phi_4 e^{-J} ) -  e^{J} ( \phi_1 e^J + \phi_2 e^{J} + \phi_3 e^{-J} + \phi_4 e^{-J} ) }\\
     &= \phi_3 \parens*{\phi_1 (1-e^{2J})  +\phi_2 (e^{-2J} - e^{2J}) + \phi_4 (e^{-2J} -1) }\leq 0\\
     \end{align*}
    \begin{align*}
      &\phi_4 e^{J \hat{a}_4 } Z_b  - \phi_4 e^{J \hat{b}_4}Z_a \\
     &= \phi_4\parens*{ e^{-J} ( \phi_1 e^J + \phi_2 e^{-J} + \phi_3 e^{J} + \phi_4 e^{-J} ) -  e^{-J} ( \phi_1 e^J + \phi_2 e^{J} + \phi_3 e^{-J} + \phi_4 e^{-J} ) }\\
     &= \phi_4 \parens*{\phi_2(e^{-2J} -1) + \phi_3 (1-e^{-2J}) }\\
     &=\phi_1 (1-e^{-2J}) (\phi_3 - \phi_2) \geq 0
 \end{align*}
 Thus \cref{ineq:dobrushin edge case} becomes
\begin{equation} \label{ineq:dobrushin final}
   -\phi_3 \parens*{\phi_1 (1-e^{2J})  +\phi_2 (e^{-2J} - e^{2J}) + \phi_4 (e^{-2J} -1) } \leq J ( \phi_1 e^J + \phi_2 e^{-J} + \phi_3 e^{J} + \phi_4 e^{-J} ) ( \phi_1 e^J + \phi_2 e^{J} + \phi_3 e^{-J} + \phi_4 e^{-J} )  
\end{equation}
 %\[ \]
Note that, by 1-Lipschitz of $\tanh,$  
\[\frac{e^{2J}-e^{-2J}}{(e^J+e^{-J})^2  } = \frac{e^{2J} - 1 }{e^{2J} + 1 }=\frac{1-e^{-2J}}{1+e^{-2J}  }=\frac{e^J - e^{-J} }{e^J + e^{-J} }\leq J\]
thus 
\begin{tabular}{ccc}
     $\phi_3 \phi_1 (e^{2J}-1) \leq \phi_3 \phi_1 J (e^{2J}+1)$ & $\phi_3 \phi_2 (e^{2J}-e^{-2J}) \leq \phi_3 \phi_2 J (e^{J}+ e^{-J})^2$  & $\phi_3 \phi_4 (1-e^{-2J}) \leq \phi_3 \phi_4 J (1+e^{-2J})$ \\
\end{tabular}
Summing these inequalities together, we have:
\begin{align*}
    \text{LHS}(\ref{ineq:dobrushin final})  &\leq J \parens*{\phi_3 \phi_1  (e^{2J}+1) + \phi_3 \phi_2  (e^{J}+ e^{-J})^2 + \phi_3 \phi_4  (1+e^{-2J})} \\
    &\leq J \parens*{\phi_3 \phi_1  (e^{2J}+1) + \parens{\phi_3 \phi_2  (e^{2J}+ e^{-2J}) + \phi_2^2 + \phi_3^2} + \phi_3 \phi_4  (1+e^{-2J})} \\
    &\leq J ( \phi_1 e^J + \phi_2 e^{-J} + \phi_3 e^{J} + \phi_4 e^{-J} ) ( \phi_1 e^J + \phi_2 e^{J} + \phi_3 e^{-J} + \phi_4 e^{-J} )
\end{align*}
This finish the proof.
 \end{proof}
 \end{comment}
%\Huy{Shorter alternative proof} 
\begin{proof}
Without loss of generality, assume that $J>0$. Let $x\sim P$ be distributed on $\mathbb{S}_n$. We want to bound $d_{TV}(e^{J\langle x,a\rangle}*P, e^{J\langle x,b\rangle}*P)$. Based on the definition of the total variation distance, what we want to show is that %we want to show
\[
\mathbb{E}[|e^{J\langle x,a\rangle}/\mathbb{E}[e^{J\langle x,a\rangle}]-e^{J\langle x,b\rangle}/\mathbb{e}[e^{J\langle x,b\rangle}]|] \le 2\kappa J.
\]
Observe that $J|\langle x,a\rangle -\langle x,b\rangle| \le 2\kappa J$. Hence, the above inequality is implied by the following: For all $(u,v) \sim \mu$ where $u,v>0$ and $e^{-2\kappa J}\le u/v\le e^{2\kappa J}$ almost surely, 
\[
\mathbb{E}|u/\mathbb{E}u-v/\mathbb{E}v| \le 2\kappa J.
\]
Fixing $\mathbb{E}u=\alpha,\mathbb{E}v=\beta$, and optimizing over $u,v$ subject to these constraints, noting that $\mathbb{E}\abs{u/\alpha-v/\beta}$ is convex in $u,v$ and the only extreme points over the feasible region of $u,v$ are when $u/v\in \{e^{\pm 2\kappa J}\}$ almost surely. Thus, we can assume that $u/v \in \{e^{\pm 2 \kappa J}\}$. Then there is a random variable $\lambda$ such that $(\lambda u,\lambda v)\in \set{(e^{\kappa J},e^{-\kappa J}),(e^{-\kappa J},e^{\kappa J})}$. Let $(u',v')=\lambda(u,v)$. Then 
\[
\mathbb{E}|u/\mathbb{E}u-v/\mathbb{E}v| = \mathbb{E}_{\lambda*\mu}|u'/\mathbb{E}u'-v'/\mathbb{E}v'|.
\]
Hence, we have reduced the problem to a distribution on two spins $\{\pm 1\}$, i.e. to show 
\[
\lambda \left|\frac{e^{\kappa J}}{\lambda e^{\kappa J}+(1-\lambda) e^{-\kappa J}}-\frac{e^{-\kappa J}}{\lambda e^{-\kappa J}+(1-\lambda) e^{\kappa J}}\right| \le \kappa J,
\]
or
\[
\lambda(1-\lambda)(e^{2\kappa J}-e^{-2 \kappa J})\le \kappa J[\lambda^2+(1-\lambda)^2+\lambda(1-\lambda)(e^{2\kappa J}+e^{-2\kappa J})],
\]
which is true since for all $x\in (0,1]$,
\[
\left|\frac{e^{2x}-e^{-2x}-x(e^{2x}+e^{-2x})}{x}\right| \le 2.
\]
\end{proof}

\begin{corollary}
Let $R $ be the Dobrushin matrix of $\mu$ then $R_{i,j} \leq \abs{u_i u_j}.$
\end{corollary}

Let $Q$ be a finite set and $\mu$ be a distribution over $Q^n.$ We can view $\mu$ as a homogeneous distribution on $\binom{\Omega}{n}$ with $\Omega$ be the disjoint union of $Q_1, \dots, Q_n,$ where each $Q_i$ is a copy of $Q.$
Let the elements of $Q$ be $c_1, \dots, c_{\abs{Q}}$
The generating polynomial for $\mu$ is
\[g_{\mu} (z_{1,c_1}, \dots, z_{n,c_1},\dots, z_{1,c_{\abs{Q}}}, \dots, z_{n,c_{\abs{Q}}}) = \sum \mu(\epsilon^1, \dots, \epsilon^n) \prod_{i=1}^n  z_{i,\epsilon_i}\]
where the sum is taken over all $(\epsilon_i)\in Q^n.$


Following \cref{def:corr}, the correlation matrix $\corMat_{\mu}$ of $\mu$ is defined by
\[\corMat_{\mu} ((i,\epsilon_i),(j, \epsilon_j) ) = \begin{cases} 1 -\P{(i, \epsilon_i)} &\text{ if } j=i \text{ and } \epsilon_j = \epsilon_i \\  -\P{(i, \epsilon_i)} &\text{ if } j=i \text{ and } \epsilon_j \neq \epsilon_i  \\ \P{(j,\epsilon_j) \given (i, \epsilon_i)} - \P{(j,\epsilon_j) } &\text{ else}\end{cases} \]
where we use $\P{(j, \epsilon_j)} $ and $ \P{(j,\epsilon_j) \given (i, \epsilon_i)}$ as shorthand for $\P{x_j = \epsilon_j} $ and  $\P{x_j = \epsilon_j \given x_i = \epsilon_i} $ respectively. We also adopt the convention that if $ \P{x_i = \epsilon_i} = 0$ then $ \corMat_{\mu} ((i,\epsilon_i),(j, \epsilon_j) ) = 0$ for all $(j, \epsilon_j).$ 
%Let $\mu:Q^n \to \R_{\geq 0}$ be a distribution

For $i\in [n],$ let $Q_i: = \set*{c_k: \P{(i, c_k)} > 0 }.$  
By similar strategy as in proof of \cref{lem:weight norm} and \cref{ineq:main}, for all $i \in [n]$ and spins $c_1, c_2\in Q_i,$ 
\begin{equation} \label{ineq:row diff}
    %d_{\TV} (\Pr{ (j, \cdot)\given (i,c_1)}, \Pr{(j,\cdot)\given (i,c_2)} ) =
    \frac{1}{2}\sum_{j\neq i, c' \in Q_j} u_j\abs{\P_{\mu}{ (j,c') \given (i,c_1) }- \P_{\mu}{ (j,c') \given (i,c_2) } } \leq u_i \norm{u_{-i}}_2^2\alpha_i^{-1}
\end{equation}
with $\alpha_i = 1- \norm{u_{-i}}_2^2.$

This gives a bound on the difference between rows of correlation matrix. To relate row difference to spectral norm, we need to following lemma.
\begin{lemma} \label{lem:row diff to spectral norm}
%Suppose $\mu: [n] \to [q]$ is a $q$-spin model.
%Suppose $Q_1, \dots, Q_n$ are finite sets. Consider distribution $\mu: Q_1 \times \dots \times Q_n \to \R_{\geq 0}.$
Suppose
there exists $C_i \geq 0$ and vector $u\in \R_{\geq 0}^n$ s.t. 
for all vertex $i \in [n]$ and spins $c_1, c_2\in Q_i,$ 
\begin{equation}
    %d_{\TV} (\Pr{ (j, \cdot)\given (i,c_1)}, \Pr{(j,\cdot)\given (i,c_2)} ) =
    \frac{1}{2}\sum_{j\neq i, c' \in [q]} u_j\abs{\P{ (j,c') \given (i,c_1) }- \P{ (j,c') \given (i,c_2) } } \leq C_i u_i 
\end{equation}
then $\norm{\diag(\vec{\alpha}) \corMat_{\mu}}_{2} \leq \max_{i=1}^n \alpha_i (1+C_i) $ where $\vec{\alpha} = (\underbrace{\alpha_1, \dots, \alpha_n, \dots, \alpha_1, \dots, \alpha_n}_{\abs{Q} \text{ times}}).$ %$\vec{\alpha} = (\underbrace{\alpha_1,\cdots, \alpha_1}_{\abs{Q_1} \text{ times}},\dots, \underbrace{\alpha_n,\cdots, \alpha_n}_{\abs{Q_n} \text{ times}}) $
\end{lemma}
\begin{comment}
\begin{claim} \label{claim:row difference to norm}
If $\sum_c v_c = 0$ and $A$ has $\frac{1}{2}\norm{A_{c_1, \cdot} - A_{c_2, \cdot}}_1 \leq C$ then $\norm{v A}_1 \leq C \norm{v}_1.$
\end{claim}
\begin{proof}
Let $Q^+:= \set*{c \given v_c \geq 0}.$
Since $\sum_c v_c = 0,$ for $c\in Q^+$ and $c'\not\in Q^+,$ we can assign weight $r_{c,c'} \geq 0$ s.t. $\sum_{c'\not\in Q^+} r_{c,c'} = v_c$ and $\sum_{c \in Q^+} r_{c,c'} = - v_{c'}.$
\begin{align*}
    \norm{\sum_c v_c A_{c, \cdot}}_1 &= \norm{\sum_{c: v_c \geq 0, c': v_c < 0} r_{c,c'}  A_{c, \cdot}-A_{c', \cdot}}_1\\
    &\leq \sum_{c: v_c \geq 0, c': v_c < 0} r_{c,c'}  \norm{A_{c, \cdot}-A_{c', \cdot}}_1\\
    &\leq 2C \sum_{c: v_c \geq 0, c': v_c < 0} r_{c,c'} \\
    &\leq 2C \sum_{c: v_c \geq 0} v_c\\
    &=  2C \norm{v}_1/2
    &= C \norm{v}_1
\end{align*}
\end{proof}
\end{comment}
\begin{proof}
Let $A = \diag(\vec{\alpha}) \corMat_{\mu},$ $D =  \diag(\P{(i,c)})_{i,c}$ and $U = \diag(u_i)_{i,c}.$
Let $\lambda$ and $\vec{v}$ be the largest eigenvalue of $A$ and its corresponding left eigenvector i.e. $\vec{v} A = \lambda \vec{v}.$ If $\lambda = 0$ then we are done. From now on, we assume $\lambda \neq 0.$ 

We first argue that $\sum_{c \in Q_i} v_{i,c} = 0. $ Let $\textbf{1}_i$ be the vector that is $1$ on entries $(i,c)$ for $c\in Q_i$ and is $0$ other wise. Then $ \textbf{1}_i D $ is a left eigenvector of $A$ with corresponding eigenvalue zero, which is different from $\lambda$, so $\vec{v}$ is orthogonal to $\textbf{1}_i D $ wrt the bilinear form $\langle \cdot, D^{-1} \cdot \rangle.$ As a result, $\langle \textbf{1}_i, v\rangle = 0$ as desired.

Next, let $A': =A U.$ We will show that for $i \in [n]$ and any distinct $c_1, c_2 \in Q_i:$ 
\[\norm{A'_{(i,c_1), \cdot} - A'_{(i,c_2), \cdot}}\leq 2 \alpha_i (1+C_i) u_i\]
Note that \[ \abs{A'{(i,c_1), (i,c)} - A'_{(i,c_2), (i,c)}} =  \alpha_i \abs{\P{(i,c) \given (i,c_1)} -  \P{(i,c) \given (i,c_2)}} u_i = \begin{cases} \alpha_i u_i &\text{ if } c \in \set*{c_1, c_2} \\ 0 &\text{ else }\end{cases}\]
Thus
\begin{align*}
    \norm{A'_{(i,c_1), \cdot} - A'_{(i,c_2), \cdot}}
    &= \sum_c \abs{A'_{(i,c_1), (i,c)} - A'_{(i,c_2), (i,c)}} + \sum_{j\neq i, c} \abs{A'_{(i,c_1), (j,c)} - A'_{(i,c_2), (j,c)}}\\
    &= 2 \alpha_i u_i + \alpha_i \sum_{j\neq i, c}\abs{\P{ (j,c') \given (i,c_1) }- \P{ (j,c') \given (i,c_2) } } u_j\\
    &= 2 \alpha_i u_i(1+ C_i)
\end{align*}
Next, we show that
$\norm{\vec{v} A U}_1 \leq C' \norm{\vec{v} U}_1$ with $C' =\max_{i=1}^n \alpha_i (1+C_i),$ and conclude that $\lambda \leq C'.$ 
For $i\in [n]$ let $Q_i^{+}$ be the set of spin $c$ where $v_{i,c} \geq 0$ and let  $Q_i^- := [q] \setminus Q_i^{+}.$ Since $\sum_{i,c} v_{i,c} = 0,$ for $c\in Q_i^+$ and $c'\not\in Q_i^+,$ we can assign weight $r^i_{c,c'} \geq 0$ s.t. $\sum_{c'\not\in Q_i^+} r^i_{c,c'} = v_{i,c}$ and $\sum_{c \in Q_i^+} r^i_{c,c'} = - v_{i,c'}.$ %Note that $\sum_{c \in Q_i^+} \abs{v_{i,c}} = \norm{v}$
Therefore
\begin{align*}
    \norm{v A'}_1 
    &= \sum_{j,c} \abs{\sum_{i,c'}  v_{i,c'}  A'_{((i,c'),(j,c)}}\\
    &=\sum_{j,c} \abs{\sum_{i,c_1 \in Q_i^+, c_2 \in Q_i^-}  r^i_{c_1,c_2}  \parens{A'_{((i,c_1),(j,c)}- A'_{((i,c_2),(j,c)}} }\\
    &\leq \sum_{i,c_1 \in Q_i^+, c_2 \in Q_i^-} r^i_{c_1, c_2} \norm{A_{(i,c_1), \cdot}- A_{(i,c_2), \cdot}}_1\\
    &\leq 2  \sum_{i,c_1 \in Q_i^+, c_2 \in Q_i^-} r^i_{c_1, c_2} \alpha_i u_i(1+ C_i)
    \leq 2C' \sum_{i, c \in Q_i^+} v_{i,c} u_i
    =C' \sum_{i,c\in[q]} u_i \abs{v_{i,c}}
    = C' \norm{\vec{v} U}_1
\end{align*}
as desired. 
% Fix $i, j \neq i.$ Using $ \sum_{c \in [q]} v_{i,c} = 0,$ we have
% \begin{align*}
%     \sum_c  v_{i,c}  \parens*{\P{(j,\cdot)\given (i,c)} - \P{(j,\cdot)}}\\
%     &\leq 
% \end{align*}
\end{proof}

Combining \cref{ineq:row diff} with \cref{lem:row diff to spectral norm}, we have the desired bound $\norm{\diag(\vec{\alpha}) \corMat_{\mu}}_{2} \leq 1.$ \cref{lem:multi spin}  and \cref{thm:multi spin} then follows from similar argument as in \cref{sec: reduce to rank 1,sec:MLSI-Ising}. We leave the details to \cref{sec:appendix}.
